A Game-theoretic Framework for Privacy-preserving Federated Learning

In federated learning, benign participants aim to optimize a global model collaboratively. However, the risk of \textit{privacy leakage} cannot be ignored in the presence of \textit{semi-honest} adversaries. Existing research has focused either on designing protection mechanisms or on inventing attacking mechanisms. While the battle between defenders and attackers seems never-ending, we are concerned with one critical question: is it possible to prevent potential attacks in advance? To address this, we propose the first game-theoretic framework that considers both FL defenders and attackers in terms of their respective payoffs, which include computational costs, FL model utilities, and privacy leakage risks. We name this game the federated learning privacy game (FLPG), in which neither defenders nor attackers are aware of all participants' payoffs. To handle the \textit{incomplete information} inherent in this situation, we propose associating the FLPG with an \textit{oracle} that has two primary responsibilities. First, the oracle provides lower and upper bounds of the payoffs for the players. Second, the oracle acts as a correlation device, privately providing suggested actions to each player. With this novel framework, we analyze the optimal strategies of defenders and attackers. Furthermore, we derive and demonstrate conditions under which the attacker, as a rational decision-maker, should always follow the oracle's suggestion \textit{not to attack}.

==> 06-Various_Settings.tex <==
\section{General Framework}
For the single-step game, we aim at finding a set of strategies achieving Nash equilibrium. For the repeated game, we aim at designing a learning strategy that converges to an approximate equilibrium. 




\subsection{The Basic Framework}

\begin{itemize}
    \item client $k$ selects a protection extent $\Delta_k$, and then upload the protected parameter to the server;
    \item a semi-honest attacker determines the attacking extent $\gamma_k$ for inferring the data set based on the released parameter.
\end{itemize}




\subsection{No-Regret Dynamics}
Algorithm design could also refer to the work "Fast Federated Learning by Balancing
Communication Trade-Offs".



For dynamic game, the approaches used in the literature include





Refer to lecture $17$ of Tim Roughgarden's game theory course.
This setting considers \textit{repeated game}, and show that a no-regret algorithm converges to correlated equilibrium.


Now we introduce the detailed design approach of the no-regret algorithm for the dynamic game. The following definitions follow the work \cite{kearns2014mechanism}.

\begin{definition}[Mechanism]
A mechanism $\calM: \calU^{K+1}\rightarrow \Delta\mathbb R^{K+1}$ is a function from a profile of payoff functions to a probability distribution over $\mathbb R^{K+1}$.
\end{definition}

\begin{definition}[The vector of payoff functions]
Let $\mathbf u = (u_1, u_2, \cdots, u_{K+1})$ be a profile of utilities.
\end{definition}

First, we should explain the word "joint differential privacy". 

\begin{definition}[$\gamma$-sensitive]
 A game is $\gamma$-sensitive if a player's choice of action affects any other player's payoff by at most $\gamma$. 
\end{definition}

In our setting, the choice of client $k$ about $\Delta_k$ will affect other player's payoff.

At each step, each player follows a no-regret algorithm. Then according to the following theorem, we know that it converges to the correlated Nash-equilibrium.
\begin{theorem}[Theorem $5$ of \cite{kearns2014mechanism}]
If the maximum regret of each player is at most $\alpha$, then the correlated action distribution $\prod_S$ is an $\alpha$-approximate coarse correlated equilibrium.
\end{theorem}

In our setting, at each step, all players select their actions simultaneously. Then they receive the utilities, and make decisions according to the no-regret algorithms separately.


\subsection{The Algorithm}
In the full information setting, the algorithm uses the \textit{reward} of each action to update the weight of each action;
In the partial information setting, the algorithm uses the \textit{UCB} of each action to update the weight of each action.






\begin{algorithm2e}[t]
    \caption{Learning Algorithm in Unknown Games}
    \label{alg: block}
    \textbf{input}: $\xi_t(a)$ \\
    \For{$t=1, 2 \ldots$}{
    $\rho_t(a) = e^{-\eta_t\tilde L_{t-1}(a)}/\sum_{a'}e^{-\eta_t\tilde L_{t-1}(a')}, \forall a$.\\
    $\epsilon_t(a) = \min\{\frac{1}{2K}, \frac{1}{2}\sqrt{\frac{\ln K}{tK}}, \xi_t(a)\}$.
    $\tilde\rho_t(a) = (1 - \sum_{a'}\epsilon_t(a'))\rho_t(a) + \epsilon_t(a).$\\
    Sample action $A_t$ according to distribution $\tilde\rho_t$.\\
    Observe the feedback $l_t(A_t)$.\\
    $\tilde l_t(a) = \frac{l_t(a)}{\tilde\rho_t(a)}\one\{a = A_t\}, \forall a$.\\
    $\tilde L_t(a) = \tilde L_{t-1}(a) + \tilde l_t(a)$.
    }
\end{algorithm2e}

Note that the privacy leakage $\epsilon_{p,t}$ at each round $t$ is bounded. There exist two constants $C_1$ and $C_2$, satisfying that $\epsilon_{p,t}\in [C_1, C_2]$.

The property of the expected reward at round $t$. Assume that the protection extent of the client is rather large at round $t$, then the aggregated parameter is not good. This might affect the model payoff at round $t+1$. The action at one round might affect the reward at the next round. Consider the semi-honest attacker, the expected payoff (expected reward) of the defender could be regarded as being corrupted, and the amount of corruption at each round ranges between $C_1$ and $C_2$. This corresponds to the adversarial setting with 







\section{Some ideas}
We could consider many settings. 
For example, in the case we do not know about the cost of the adversary, we could assume that the cost of the attacker is at most his privacy gain at each step (which might correspond to zero-sum.) Then we could analyze the strategy of the defender in worst case, in average case. 















\subsection{Malicious Adversary}

\begin{itemize}
    \item client $k$ selects a protection extent $\Delta_k$, and then upload the protected parameter to the server; $w_k^{\calO}\rightarrow w_k^{\calD}$.
    \item a semi-honest attacker determines the attacking extent $\gamma_k$ for inferring the data set based on the released parameter. $w_a^{\calO}\rightarrow w_a^{\calD}$.
\end{itemize}


$\term_1$ represents the improvement of model utility due to aggregation without using any protection approach, which depends on the attacking approach and is independent of the protection mechanism;
$\term_3$ represents the performance decrease due to the poisoning of the adversary, which is regarded as an optional term.





==> 08-Randomization_Mechanism.tex <==
% \section{Example: Randomization Mechanism}


% \begin{definition}[Cost of adversary]
% Let $t(\gamma_k)$ represent the time cost of the attacking approach $f$, and $c(\gamma_k)$ represent the corresponding payoff expenditure, which is defined as follows:
% \begin{equation}
% c(\gamma_k)=\left\{
% \begin{array}{cl}
% \eta\cdot t(\gamma_k), &  t(\gamma_k) \text{ is polynomial.}\\
% \infty,  &  t(\gamma_k) \text{ is exponential.}\\
% \end{array} \right.
% \end{equation}
% \end{definition}

% % \begin{lem}
% % Assume that the adversary uses a total of $t^2$ rounds for attacking the client, then we have $g_p(w_{k}, T_{K+1}) = T_{K+1}^2\cdot ||w_{k} - w^*||$.
% % \end{lem}
% %\begin{proof}


% Let $T_{K+1}$ represent the time cost of player $K+1$, who is an attacker. Let $T_u$ represent the time complexity of the attacking algorithm used by the attacker. Let
% \begin{equation}
% c(T)=\left\{
% \begin{array}{cl}
% T, &  T< T_u\\
% T_u,  &  T\ge T_u\\
% \end{array} \right.
% \end{equation}

% % Note that $\log(c(T_{K+1}))$ illustrates that the learning rate is fast initially, and then decay until the algorithm converges. 


% It implies that 
% \begin{itemize}
%     \item the smaller distance between the exposed parameter $w_{k}$ and the real parameter $w^*$ is, then the more privacy information the attacker gains;
%     \item the longer the attacking time is, then the more information the attacker gains.
% \end{itemize}

% \red{
% What is the goal of the oracle? Maximize the social welfare? What is the definition of the social welfare?
% }

==> 09-Payoff_of_the_defender.tex <==

% \section{The Oracle}
% The oracle provides upper bound and lower bound using $\Delta_k$ and $C_a$. He/she informs the upper bound and lower bound of the payoff matrix. The oracle provides correlation probability matrix. The player decides whether to follow.

% \subsection{payoff Bounds}

% The oracle provides an estimation of the payoff of the players, according to the machine learning theory \cite{kingma2014adam}. Assume that $\Delta_i\in\{\epsilon^0, \epsilon, \epsilon^2, \epsilon^3, \cdots, \delta\}$ for any defender $i$. Then the payoff matrix is illustrated as follows, where $M = \log_2(\frac{1}{\delta})$.

% \begin{figure}[h]
% \centering
% \includegraphics[width = 0.95\columnwidth]{Fig_payoff_Matrix.png}
% \caption{payoff Matrix}
% \label{fig: flowchart}
% \end{figure}




% \subsection{Correlation Probability Matrix}
% The oracle also provides the players the correlation probability matrix, as illustrated in \ref{table: correlation_prob_matrix}.

% \begin{table*}[!htp]
% \footnotesize
%   \centering
%   \setlength{\belowcaptionskip}{15pt}
%   \caption{Correlation Probability Matrix}
%   \label{table: correlation_prob_matrix}
%     \begin{tabular}{ccccc}
%     \toprule
%      & $C_1$ & $C_2$ & $\cdots$ & $C_M$\cr
%     \midrule\
% $\Delta_1$ & $p(\Delta_1, C_1)$	 & $p(\Delta_1, C_2)$ & $\cdots$ & $p(\Delta_1, C_N)$\cr
% $\Delta_2$ & $p(\Delta_2, C_1)$ &  $p(\Delta_2, C_2)$ & $\cdots$ & $p(\Delta_2, C_N)$\cr
% $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$\cr
% $\Delta_M$ & $p(\Delta_M, C_1)$ &  $p(\Delta_M, C_2)$ & $\cdots$ & $p(\Delta_M, C_N)$\cr
%     \bottomrule
%     \end{tabular}
% \end{table*}
